BigMac: Breaking the Pareto Frontier of Compute and Memory in Multimodal LLM Training

Training multimodal large language models (MLLMs) is challenged by both model and data heterogeneity. Existing systems redesign the training pipeline to address these challenges, but remain bound by a Pareto frontier between compute and memory efficiency, improving one only at the expense of the other. We present BigMac, a new training pipeline for multimodal LLMs. The core idea of BigMac is to elegantly nest the encoder and generator computation into the original LLM pipeline, forming a dependency-safe nested pipeline structure. With this design, BigMac reduces the activation memory complexity of the encoder and generator to O(1) while keeping the activation memory complexity of the LLM unchanged. At the same time, it achieves the same computational efficiency as the idealized setting with unlimited memory. As a result, BigMac breaks the Pareto frontier between computational efficiency and memory usage, enabling simultaneous optimization of both computation and memory in MLLM training. We evaluate BigMac on multiple MLLMs and training workloads. Experimental results show that BigMac achieves a 1.08$\times$-1.9$\times$ training speedup over baseline systems while maintaining stable memory usage as batch size increases.

==> Makefile <==
NAME=paper

TARGET=$(NAME)

all: $(TARGET).pdf

quick: Makefile *.tex sections/*.tex *.bib
	pdflatex  $(TARGET).tex
# 	rm -f *.aux *.log *.out *.bbl *.blg *~ *.bak *.ps *.synctex.gz
	if which xdg-open 1>/dev/null 2>&1; then \
		xdg-open $(TARGET).pdf; \
	else \
		open -a Preview $(TARGET).pdf & \
	fi

$(TARGET).pdf: Makefile *.tex sections/*.tex *.bib
	pdflatex  $(TARGET).tex
	-bibtex --min-crossrefs=100    $(TARGET)
	pdflatex  $(TARGET).tex
	pdflatex  $(TARGET).tex
# 	rm -f *.aux *.log *.out *.bbl *.blg *~ *.bak *.ps *.synctex.gz
	if which xdg-open 1>/dev/null 2>&1; then \
		xdg-open $(TARGET).pdf; \
	else \
		open -a Preview $(TARGET).pdf & \
	fi

clean:
# 	rm -f *.aux *.log *.out *.bbl *.blg *~ *.bak *.ps $(TARGET).pdf *.synctex.gz


==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
This is discussion.

==> sections/implementation.tex <==
\section{Implementation}
\label{sec:implementation}

This is implementation.

==> sections/overview.tex <==
\section{\sysname Overview}
\label{sec:overview}

\sysname consists of two main components: the \sysname pipeline scheduler and the \sysname pipeline executor.
The pipeline scheduler is responsible for determining the optimal scheduling of
microbatches across different modules, while the pipeline executor manages the execution of the
scheduled microbatches on the underlying training framework.

\parabf{Pipeline scheduler.}
The \sysname pipeline scheduler is designed to optimize microbatch scheduling across the three
MLLM modules: the modality encoder, the LLM, and the modality generator. Its key idea is to disaggregate scheduling across modules while preserving the logical dependencies required for correct execution.
To this end, it divides pipeline operators into two categories: compute operators and communication operators.
For compute operators, the scheduler preserves the execution order of LLM operators under a user-specified LLM schedule
(e.g., interleaved 1F1B), while disaggregating the encoder and generator from the monolithic pipeline and
nesting their operators within the LLM schedule. This nested design achieves both optimal compute efficiency and optimal memory efficiency.
For communication operators, the scheduler is aware of the computation patterns and orchestrates data transfers to
guarantee data availability for compute operators while overlapping communication with computation whenever possible to further improve training efficiency.


\parabf{Pipeline executor.}
\sysname's pipeline executor is responsible for executing the microbatches according to the schedule determined by the pipeline scheduler.
It is architecturally disaggregated from the underlying training frameworks,
allowing it to be readily integrated with diverse systems. For example, users can employ Megatron-LM~\citep{x}
for LLM training and Torch-FSDP~\citep{y} for modality encoder and generator training,
while still benefiting from \sysname's efficient pipeline scheduling and execution. 
This disaggregated design extends beyond framework integration to parallelism strategy selection:
because the three MLLM modules are trained with different frameworks, \sysname naturally supports
different parallelization strategies for each. For instance, users may apply data parallelism to the modality
encoder and generator, while adopting hybrid parallelism (e.g., expert parallelism and context parallelism)
for the LLM. By disaggregating pipeline execution from both framework choice and module-level parallelization,
\sysname enables users to combine the strengths of their preferred training stacks while still achieving high MLLM training performance.


==> sections/related.tex <==
\section{Related Work}
\label{sec:related}
This is related work.
